Accelerating OTA Circuit Design: Transistor Sizing Based on a Transformer Model and Precomputed Lookup Tables

Device sizing is crucial for meeting performance specifications in operational transconductance amplifiers (OTAs), and this work proposes an automated sizing framework based on a transformer model. The approach first leverages the driving-point signal flow graph (DP-SFG) to map an OTA circuit and its specifications into transformer-friendly sequential data. A specialized tokenization approach is applied to the sequential data to expedite the training of the transformer on a diverse range of OTA topologies, under multiple specifications. Under specific performance constraints, the trained transformer model is used to accurately predict DP-SFG parameters in the inference phase. The predicted DP-SFG parameters are then translated to transistor sizes using a precomputed look-up table-based approach inspired by the gm/Id methodology. In contrast to previous conventional or machine-learning-based methods, the proposed framework achieves significant improvements in both speed and computational efficiency by reducing the need for expensive SPICE simulations within the optimization loop; instead, almost all SPICE simulations are confined to the one-time training phase. The method is validated on a variety of unseen specifications, and the sizing solution demonstrates over 90% success in meeting specifications with just one SPICE simulation for validation, and 100% success with 3-5 additional SPICE simulations.

==> sec/DPSFG_pseudocode.tex <==

\small
\begin{algorithm*}[t]
\vspace{-0.5cm}
\caption{Automated DP-SFG Generation for single phase analog circuits}
\label{algo:dpsfg}
\begin{multicols}{2}
\begin{algorithmic}[1]
\State \textbf{Input:} Netlist of circuit components (RCs, transitors, etc.)
\State \textbf{Output:} DP-SFG of the circuit
\State $V \gets \text{All terminals in the netlist as nodes}$  \label{algo1:init_begin}
\State $D_{nc} \gets \text{Initialize node-component dictionary including parasitics}$
\State $D_{cn} \gets \text{Initialize component-node dictionary including parasitics}$
\State $T_{n} \gets \text{All transistors and corresponding terminals}$ \label{algo1:init_end}

\Statex \textit{// \textbf{Step 1}: Initialization of auxiliary nodes}
\For{node $n$ in $D_{nc}$} \textit{// Iterate over all nodes} \label{algo1:step1_begin}
    % \If{$n$ is not connected to $Ground$}
        % \State $C \gets$ All components $c$ connected to $n$
        % \If {$\nexists$ no voltage in $C$}        
    %         \State $F_{aux}[n] \gets 1$ \textit{//node $n$ auxiliary flag assigned 1}
    %         \State Create auxiliary node $\Ddot{n}$
    %         \State Create edge $(\Ddot{n}, n)$ = driving-point impedance at $n$
    %     \EndIf
    % \EndIf
    \If{ $n \not =$ ground \textbf{or} connected to voltage source}   
        \State $F_{aux}[n] \gets 1$; Create auxiliary node $\hat{n}$
        \State Add edge $(\hat{n}, n)$; weight = driving-point impedance at $n$
    \EndIf    
\EndFor \label{algo1:step1_end}
\Statex \textit{// \textbf{Step 2}: Adding branches due to passive components}
\For{component $c$ connected between terminals $i, j \in D_{cn}$} \label{algo1:step2_begin}
    \State $G_c \gets$ admittance of component $c$ 
    \If {node $t \in \{i,j\}$ connects to an auxiliary source node $\hat{t}$}
    \State Add an edge from the other terminal to $\hat{t}$ with weight $G_c$
    \Else
    \State Add an edge from $i$ to $j$ with weight $G_c$ 
    % \redHL{Not clear. These are directed edges (I think) - so why $i$ to $j$, and not $j$ to $i$. The two terminals of a resistor are indistinguishable in terms of direction. \textbf{I did it according to the terminals ...like PLUS terminal to MINUS terminal of Resistors from netlist convention.....to be exact Higher potential to lower} {\em How do you know the potential? You have not solved the circuit and you don't know any voltages.}}
    \EndIf
    % \State {\em Is this what you want to say? \textbf{The edge should be from the non-aux node to the auxnode } OK now?yes YES (If so, pl delete this comment and remove the lines below. If not, please let me know how to correct it. As you will see, this is much more human-readable. The goal of pseudocode is to explain an algorithm clearly, rather than to be semantically correct and exhaustive wrt listing all if-then-else cases. Please use this guidance to adjust Step 3 (I have not seen your most recent version. FYI, I am landing soon and may be offline till ~10pm CT. Meanwhile, can you look at how I have rewritten Step 1, and write Steps 2 and 3 in that way? I first explain the {\em principle} and then go to the example of Fig. 2 to provide a particular case. Thanks. Also: trans-conductance $\rightarrow$ transconductance (``trans'' is not a stand-alone word (I can hyphenate ``stand-alone'' because ``stand'' and ``alone'' are both valid words.). Pl. search for all hyphenated words and fix.} OK PROF
    
    % \State $F_{aux}[s] == 1$ ? $(d, \hat{s})$ $\gets$ $G_c$ 
    % \State $F_{aux}[d] == 1$ ? $(s, \hat{d})$ $\gets$ $G_c$ 
    %\State If neither node is auxiliary, create edge $(s, d)$ $\gets$ $G_c$
\EndFor \label{algo1:step2_end}

\Statex\textit{// \textbf{Step 3}: Adding branches due to transconductance $g_m$}

\For{$t$ in $T_n$} \textit{// Iterate over all transistors} \label{algo1:step3_begin}
    \Statex \textit{// $I_d[t]$: Drain current of t; $g$: Gate; $s$: Source, $d$: Drain}

    \If{$V_{gs} \neq 0$}
        \If{transistor $t$ is NMOS}
            \State For node $i$, $j$  in $\{s,d\}$ terminals:
            \If{Voltage at node $i \propto I_d[t]$}
                \State Add edges from $i$ to $\hat{i}$ with weight $-g_m$ 
                \State Add an edge from $i$ to $\hat{j}$ with weight $+g_m$ 
            \Else  
                \State (Same as above, but negate the edge weights)
            \EndIf
            \State Add an edge from $g$ to $\hat{d}$ with weight $-g_m$ 
            \State Add an edge from $g$ to $\hat{s}$ with weight $+g_m$ 
        \Else \textit{// For PMOS transistors}
            \State (Same as above, but exchange ``then'' and ``else'')
        \EndIf
\EndIf
\EndFor \label{algo1:step3_end}


% \For{$t$ in $T_n$} \textit{// Iterate over all transistors}
%     \If{$V_{gs} \neq 0$}
%         \If{transistor $t$ is NMOS}
%             \State For node $t$ in \{s,d,g\} terminals:
%             \If{Voltage at node $t \propto I_d[t]$}
%                     \State $(t, \hat{x}) \gets (I_d[t] \propto V_{x} \text{ and } x \neq g) \ ? \ -g_m : +g_m$
%                     \State $(x, \hat{y}) \gets (I_d[t] \propto V_{x}) \ ? \ +g_m : -g_m$
%                 \Else
%                     \State $(g, \hat{d}) \gets -g_m$
%                     \State $(g, \hat{s}) \gets +g_m$
%                 \EndIf
%         \Else
%             \State For PMOS transistors, the logic for edge creation would be opposite.
%         \EndIf
% \EndIf
% \EndFor





\end{algorithmic}
\end{multicols}
\vspace{-0.3cm}
\end{algorithm*}
\normalsize


